A study of Neural networks point source extraction on simulated Fermi/LAT Telescope images

Astrophysical images in the GeV band are challenging to analyze due to the strong contribution of the background and foreground astrophysical diffuse emission and relatively broad point spread function of modern space-based instruments. In certain cases, even finding of point sources on the image becomes a non-trivial task. We present a method for point sources extraction using a convolution neural network (CNN) trained on our own artificial data set which imitates images from the Fermi Large Area Telescope. These images are raw count photon maps of 10x10 degrees covering energies from 1 to 10 GeV. We compare different CNN architectures that demonstrate accuracy increase by ~15% and reduces the inference time by at least the factor of 4 accuracy improvement with respect to a similar state of the art models.

==> description/descrip.tex <==
\section{Problem description}
As noticed above, the images in the GeV band can be affected by strong contribution of diffuse background. In what below we describe the algorithm able to isolate point-like sources in astrophysical maps.

%are subject to the noise of a completely different nature. Our task is to create an algorithm to identify sources. 
To efficiently train the models we need plenty of data and the real data is not enough. In the real life we have just one sky with finite number of regions/sources. Thus we selected to use the artificial dataset. It replicates properties of the signal and background without dependence on specific prior distributions. 

\subsection{Dataset} 


The dataset contains simulated images of objects similar to the ones taken by Fermi/LAT, see e.g.~\cite{3fgl_catalogue,4fgl_catalogue} for catalogues of detected sources. In addition to images, we provide coordinates of all the point sources within those images. Such a dataset is realistic enough to test deconvolution techniques. We do not limit ourselves to high galactic latitudes with low background level, the dataset contain significant amount of images with strong galactic diffuse background contamination. 

Fermi/LAT produces images as raw count maps of photons of selected energy band detected during certain time period. We have chosen the energy range of 1--10~GeV (close to optimal Fermi/LAT sensitivity band for point-like sources) and a time span of 10 years (similar to current mission duration $\sim 12$~years). Each image corresponds to a sky segment of $10^\circ\times10^\circ$ degrees or $200\times200$ pixels. Coordinates of point sources refer to a local Cartesian system of an image with centre at its top left corner. We center the images at random positions in the sky.

To simulate this dataset, we use the Fermi tools software \cite{website:fermi-tools}. The astrophysical Diffusive Background is modeled as a sum of two standard templates (extragalactic: iso\_P8R2\_CLEAN\_v6 and galactic: gll\_iem\_v06.fits)  at corresponding sky segment. We add point sources randomly distributing them on the picture. Their brightness is sampled from the range [0.5*minimal brightness of real 3FGL catalogue sources found in the sky segment from which background was retrieved ; 1.15*maximal brightness of these real sources]. The number of the sources per image is sampled from the range [number of these real sources +-2]. Based on this data, an XML file is created and used to generate an image with the help of \textit{gtmodel} routine of Fermi tools. To make the data realistic (only integer number of photons can be observed), we replace the value in each pixel of the produced map with a value derived from a Poisson distribution with a mean equal to the value simulated for the corresponding pixel.

There are two kinds of images in the dataset. One of them is where the brightness of some sources is greater than the brightness of the background and the ones where these intensities are comparable including the ones with strong background.(Fig. \ref{fig:dataset_ex}).

\begin{figure}
    \centering
    \includegraphics[scale=0.17]{images/example_dataset.png}
    \caption{Images$\#$0 is a first type of images where the brightness of the sources is greater than the brightness of the background. Images$\#$1 shows the second type where the brightness of sources and background are comparable. Masks here stand for images where all real point sources are marked as white crosses. }
    \label{fig:dataset_ex}
\end{figure}


As far as this dataset has been generated based on the real data, it can be used for comparison of various denoising algorithms. The dataset consists of 3692 images. During the training process, 2954 of them was used for training 738 for validating and 407 for testing.
\subsection{Metrics} 
\label{desc:metrics}

In order to analyze the performance of deconvolution models a metric which allows to define the distance between the set of predicted sources (set $A$) and ground truth sources (set $B$) has to be defined. We propose this metric $dist(A,B)$ to be Chamfer Distance, introduced for 3D data analysis (e.g. for 3D Object Reconstruction in \cite{chamferDistance} ):

%We have to measure how close the predicted sources are to the real sources to analyze the model’s performance. For each predicted point $a$ (defined by its Cartesian coordinates in the image plane) the algorithm finds the nearest neighbor in the original set $B$ and sums the squared distances up. Then we sum of the distance from predicted points to original ones and the distance from ground truth sources to predicted ones. 
%\begin{equation}
%\label{eq:asym_metric}
%Dist(A, B) = \sum_{a \in A} \min_{b \in B}\|a - b\|_2    
%\end{equation}

%\begin{equation}
\begin{align}
\label{eq:metric}
& dist(A, B) = Dist(A, B) + Dist(B, A)  \\ \nonumber
& Dist(A, B) = \sum_{a \in A} \min_{b \in B}\|a - b\|_2    
\end{align}

Here $\|a - b\|_2 = \sqrt{\sum{\|a - b\|^2}}$ stands for a Euclidean norm.


To accelerate its calculations, the BallTree structure is used \cite{balltree}. 
This metric is symmetric, non-negative, continuous, and piece-wise smooth.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%We denote the set of images as $X$, $Y$ as ground truth coordinates, and $f$ as our predicting model that returns predicted source coordinates for given images. We compute the distances for each astrophysical image between predicted sources and original ones, and then we take an average.

Below we consider predicting model $f$ which acts on an image $x$ and returns predicted sources list $f(x)$. Let $y$ be the list of ground truth sources in the corresponding image $x$. In case if $x$ belongs to a collection of images $X$, a corresponding collection $Y: y\in Y$ can be considered. For a given collection of images $X$ and corresponding collection of ground-truth coordinates $Y$ we define the score of the predicting model $f$ as
\begin{equation}
\label{eq:score}
\text{score}(f,X,Y) = \frac{1}{|X|}\sum_{x, y \in X, Y} dist(y, f(x))
\end{equation}

where $|X|$ is the number of images in the considered collection $X$.  

%The sum in the above equation~\ref{eq:score} goes over all $(x;y)\in(X,Y): f(x)\neq\varnothing \mbox{ and } y\neq\varnothing$.

This metric assumes that both predicted and ground truth source sets are not empty. Otherwise,
%\todo[inline]{Sounds weird. "Otherwise" -- i.e. only if at least one of these sets is empty. Then: for each not found or falsely detected. False detection or not found could happen even if both sets are not empty, right? }
%\todo[inline,backgroundcolor=green]{This is exactly what we did... the penalizing term appears only if one of the sets is empty. If both of them are not empty, for each non-detected point we will sum the closest detected which will penalize. Chamfer distance is simply not defined when one of the sets are empty. That is why we study this case independently.}
we introduce penalizing term (\textbf{P}) to the score for each not found or falsely detected source by a fixed constant per point:

$$ P = \frac{1}{8}* H *|C| \text{, where}$$
$C$ is a non-empty set of points, and $H$ \todo[backgroundcolor=green]{done} is a size in pixels of a side of our square-image.
 \textbf{P} is used as a score when either we have a picture without point sources but some were predicted, either no point sources were predicted for an image which contain ground-true point sources.

For a more detailed analysis of errors, we will also consider the following standard metrics: F1 score and True Positive Rate(TPR) \cite{roc}.
We do not consider False Negative Rave and True Negative Rate because the number of negative elements tends to be rather large; therefore, these metrics will not work.




==> disc/disc.tex <==
\section{Discussion}

As we observe the trade-off between the time and the performance for different algorithms in our result table, we can make the following comments. 

D3PO finds less than a half of all point sources but it rarely detects false sources. Testing time appears to be extremely large due to small convergence rates. 
SExtractor shows better results than D3PO significantly improving mean metrics score over the test set. It takes nearly one forth of the second to execute for one test image. Selection of background priors, suggested by the authors, perform poorly on our data set. Its initial parameters give metric scores close to 1200. Thus, we optimize for better priors using a training set. Also, we change the threshold of the algorithm. It improves a bit as the output points tend to cluster around real sources. Thus, to improve the accuracy, one can apply DBSCAN with $\epsilon$=0.01. 

SExtractor algorithm is very sensitive to parameters. With default parameters, the metric score is close to 2000.  The optimal settings have been selected as a result of extensive optimization. 


%Empirically, it was found that the most important parameters are:
%DETECT_MAXAREA =  24  
%DETECT_MINAREA =  1.85
%DETECT_THRESH = 1.85 
%ANALYSIS_THRESH = 20000

 
The simple CNN is the first neural network approach tested. Its performance drops comparing to SExtractor while in terms of speed it outperforms the same algorithm by factor of 6. We notice that SExtractor have the same precision as CNN for f1 and TRP scores. 

YOLO improves true-positive rate and metrics variation while its F1-score is slightly worse compared to two previous approaches. Its metrics score stays close to SExtractor performance with the time execution comparable with CNN.

UNet and FoCNN succeed to improve the results further. Their overall performance is nearly the same, Unet works faster but FoCNN has a better true-positive rate. We also tested them on an extended data set getting 307 and 302 metrics scores respectively. The extended dataset was generated following the same algorithm as the  testing set. It contains 900 new samples. 




%\begin{figure}
%    \centering
%    \includegraphics[scale=0.25]{images/predict.png}
%    \caption{UNet model predictions on test data.}
%    \label{fig:predit}
%\end{figure}

The significant difference in metrics score for CNN and SExtractor might be the consequence of false positives that are situated closer to real sources in the SExtractor case. Thus, we can conclude that although SExtractor successfully detects a point source in some regions, it fails to localize them correctly.

FoCNN shows better performance on the extended data set both in terms of accuracy and performance. It contained data from the same distribution. It improves accuracy by $\approx 15 \%$ compared to SExtractor and reduces the inference time by a factor of 4.

In real life there are also extended sources, not only point ones. Our models will most likely miss them interpreting as a part of diffused background.

==> introduction/intro.tex <==
\section{Introduction}

Modern gamma-ray telescopes, e.g. Fermi/LAT~\cite{lat} or AGILE~\cite{agile} explore the sky in 0.1 -- 100~GeV energy band. \textit{These instruments are characterised by a broad field of view ($20\%$ of all sky for Fermi/LAT) and normally operate in ``sky-survey'' mode with a rare dedicated pointing observations. Direction of every detected gamma-ray photon can be reconstructed with certain energy dependent accuracy. The detected photons are
This allows creation of maps which illustrate spatial distribution of the emission in selected energy band.}\textcolor{}{
These instruments are characterised by a broad field of view ($20\%$ of all sky for Fermi/LAT) and normally operate in ``all sky-survey'' mode in which the telescope continuously scans the sky. The photons cause a response once they arrive at the detector. An incident photon result in an event that is called "count" for the corresponding sky region. These counts are summed up to form the gamma map of the sky. This map is also called observations.}

Several different-class objects can appear on a typical GeV map -- point-like galactic and extragalactic (isotropic) sources (e.g. pulsars and active galactic nuclei); extended galactic and extragalactic sources (e.g. supernova remnants and jets from nearby radio-galaxies); galactic (mainly hadronic emission from gas clouds; variable at a degree-scale, see e.g.~\citet{fermi_galdiffuse}) and extragalactic diffuse emission. Characteristic angular sizes of these sources vary from degrees (extended sources) to close to all sky scales (diffuse sources). A finite and energy dependent ($\sim 1^\circ$ at 1~GeV and $0.1^\circ$ at 100~GeV, see e.g.~\cite{lat_psf}) accuracy of the photon arrival direction reconstruction lead to the additional artificial broadening even of point-like sources. Due to this broadening extended and even point-like sources can be confused with the similar angular-scale features in galactic diffuse emission. Additional complexity arises from the low-statistics of the observed data, which becomes thus a subject of Poisson noise.


In this paper we propose a deconvolution technique which allow to detect and separate point-like sources from the diffuse component.

Since \cite{AlexNET}, neural networks have been invading different areas of research from medical image analysis by \cite{medical_nn} to jet structure analysis in the particle physics by \cite{deepadvertising}. Our neural networks do not require any additional information to output results except for the original data. Most state-of-the-art deconvolution algorithms in astrophysics imply specific parameters that should be tuned for the particular dataset characteristics. Hence, reducing the generality of the approaches. The examples can be found in the Related work section.

The deconvolution problem for point sources can be reduced to a segmentation problem with two classes: background and sources. We address the problem as a segmentation problem via Unet by \cite{unet} and via our neural net architecture. The main problem is the class imbalance as the number of background pixels four orders of magnitude times larger than the signal pixel number.

We generate our artificial dataset and define metrics to evaluate our results.  We compare these methods with classical approaches SExtractor by \cite{sxtractor1996} and D3PO by \cite{d3po} and object detection approach via YOLO by \cite{yolo}, and estimate their performance.

This article consists of seven parts. In the second part, we will analyze the literature. The third part reveals the formulation of the problem with the dataset and metric description; the fourth describes models, preprocessing methods, and training process. The quality of the models and error research in the fifth part. The sixth part is devoted to the result discussion.


==> models/models.tex <==
\section{Models} 

We search for a mapping from original astrophysical images to point source coordinates of these images. Chosen Chamfer distance  measure the quality of the introduced models.
As baselines, we choose D3PO algorithm and SExtractor. We suggest a simple neural network with four layers, UNet \cite{unet} and FoCNN as our solutions. All of them are convolution neural networks \cite{AlexNET}.

Before describing the architectures, we notice that the dataset is very unbalanced. It consists of a significantly different number of sources points and background points. The mean number of point sources per image is equal to 7 against mean number of background pixels equal to 39993. Due to class imbalance, the networks tend to output small values even for point sources. Thus, we introduce another parameter, a threshold for network output. Pixels of the output image which have values equal or greater than this threshold should be interpreted as point sources. The value of this parameter is defined through the optimization.


% Мне не нравится перенос данной секции в ридми (не справедиливо для других статей) и в результаты (там не должно быть подробного описаания моделей, хз) Или тут, или удалить (имхо)

\subsection{Images cropping}
We already introduced a threshold as one of the class imbalance acceleration technique. Second technique is images cropping. To speed up the learning process we train the models with cropped images. From image $200 \times 200$ we crop image $s \times s$ where $s$ may be various for different network architectures.

Sources are not uniformly distributed over an image, if we will crop randomly, from 2000 crops on average, only 500 will contain sources. But if a neural network during training stage receives empty $s \times s$ it will lead to small training rates. That is why additionally to threshold we implement picking randomly only a fraction of images without sources. Another technique is random sampling. With a chosen probability, we take either a sample with at least one source or a random one. Using these techniques we can control number of sources during the training process. In the Figure \ref{fig:batch} we give examples of cropping for $s = 40$.

%We crop input images from $200 \times 200$ to several $s \times s$ ones where $s$ may be various for different network architectures.
%Sources are not uniformly distributed over an image. From 2000 crops on average, only 500 contain sources.
%Thus, we use several techniques to accelerate training mitigating imbalance. \todo[backgroundcolor=green]{Added here...}We already introduced a threshold but if a neural network during training stage receives empty $s \times s$ it will lead to small training rates. That is why additionally to threshold we implement picking randomly only a fraction of images without sources. Another technique is random sampling. With a chosen probability, we take either a sample with at least one source or a random one. In the Figure \ref{fig:batch} we give examples of cropping for $s = 40$.

%\todo[inline]{Why do we need this cropping? It seems not connected to previous or next section to me. Please consider to move this section somewhere...}
%\todo[inline,backgroundcolor=green]{We explain that it is done to reduce imbalance...}

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.5]{images/batch.png}
    \caption{Examples of cropped images and masks with size 40x40 pixels. Images are again raw photon counts. Masks contain only their ground-truth point sources marked as 1-pixel white squares.}
    \label{fig:batch}
\end{figure}


\subsection{Network Architectures}
\subsubsection{Simple CNN}

Small Convolutional Neural Networks have a significant advantage over large architectures as they contain few parameters and are quickly trained. We use a small CNN with four layers (Table \ref{tab_cnn}).

This network takes an image as an input and returns an output of the same size. The sigmoid function maps output values from 0 to 1, where 1 corresponds to the presence of the source at the given pixel. To train this network, we optimize Cross-Entropy loss from \cite{Goodfellow2016}. Also, we use re-weighing of the loss function to penalize more for missing the source and less for missing background. 

\begin{center}
\begin{table}
\centering
\makebox[0pt][c]{\parbox{0.9\textwidth}
{
\begin{minipage}[b]{1.0\linewidth}\centering
 \begin{tabular}{|| c | c | c | c | c ||}
 \hline
 Layer  & KernelSize & Stride & Padding & Activation \\ [0.5ex]
 \hline\hline
 Conv. & 7x7 & 1 & 6 & ReLu \\
 \hline
 Conv. & 3x3 & 1 & 2 & ReLu \\
 \hline
FC & - & - & - & Sigmoid \\
 \hline
 \end{tabular}
\end{minipage}\hfill
}}\vspace*{2mm}
\caption{Simple CNN.}
\label{tab_cnn}
\end{table}
\end{center}



\subsubsection{UNet} 
UNet of $\cite{unet}$ is among the best neural networks for binary segmentation tasks. This architecture consists of two parts: a) encoder that reduces the dimensionality of the original image while increasing the number of channels followed by b) decoder iteratively returning encoded representation to the original image size and channel number. This architecture identifies image features of different scale, improving the quality of the result.

We tune UNet for optimal parameters for our specific problem. A detailed explanation can be found in the \hyperref[sec:app]{Appendix} section.
\begin{enumerate}
    \item Initial number of filters = 16
    \item Kernel size = 5
    \item Number of blocks = 3
\end{enumerate}

The first parameter corresponds to the number of features in the first UNet block. Each subsequent block doubles the number of features. Kernel size is the size of the kernel in the convolution layer.  The \textit{number of blocks} corresponds to the number of blocks in the Decoder and Encoder parts.

We train UNet with EarlyStopping criterion with patience equal to 3 from \cite{earlystopping}. We use Adam optimizer with the learning rate equal to 0.001. Each batch from the training set contains at least half images with no less than one source on it. Due to our image cropping, a batch consists of two parts: one half is random images, the other one contains images with at least one source.

\subsubsection{FoCNN}

Fourier transformation is widely used for denoising tasks in image processing. We combine it with a simple convolutional neural network, which takes several images as an input. Neural networks already contain non-linearity inside, but multiple inputs allow them to provide non-linear information directly. It may reduce network size without efficiency drop.

First, we apply Fourier transformation to the image, then modify a frequency domain image, and finally, return a new image via inverse Fourier transformation. We choose three different bands: 0, 14, and 18 side square cut from the center of $20 \times 20$ frequency domain image. They are fed to the neural network alongside an unedited image. The architecture can be found in Figure \ref{fig:fcnn}.


\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.23]{images/fcnn.png}
    \caption{FoCNN Architecture. The network takes a raw count photons image and its transformed versions. One skip connection is added in the middle layers. The output is a map. Its pixels greater than chosen threshold value correspond to predicted point sources. }
    \label{fig:fcnn}
\end{figure}

After a first convolution block, we concatenate the output with the original astrophysical image to preserve small details. We put these features through a second convolution block and two fully-connected layers. The last activation function is a sigmoid. The output is a vector with 400 components where each component corresponds to a pixel of $20 \times 20$ image.

We train this neural network using Adam optimizer for 50 epochs with the linear combination of cross-entropy and MSE loss.

$$\mathcal{L} = \frac{1}{N^2}\sum_{i,j} (y_{i,j} - f(x)_{i,j})^2 + 100*(-\frac{1}{N^2}\sum_{i,j} y_{i,j} \log f(x)_{i,j})$$


\begin{table}[!htb]
    
    \begin{subtable}
      
      \centering
 \begin{tabular}{|| c | c | c | c | c ||}
 \hline
 Layer  & KernelSize & Stride & Padding & Activ \\ [0.5ex]
 \hline\hline
 Conv. & 3x3 & 1 & 1 & ReLu \\
 \hline
 Conv. & 5x5 & 1 & 2 & ReLu \\
 \hline
 Conv. & 3x3 & 1 & 2 & ReLu \\
 \hline
        \end{tabular}
        
    \end{subtable}
    \bigskip
     \begin{subtable}
      \centering
        
 \begin{tabular}{|| c | c | c | c | c ||}
 \hline
 Layer  & KernelSize & Stride & Padding & Activ \\ [0.3ex]
 \hline\hline
 Conv. & 3x3 & 1 & 2 & ReLu \\
 \hline
  MaxPool. & 2x2 & None & 0 & ReLu \\
 \hline
 Conv. & 3x3 & 1 & 2 & ReLu \\
 \hline
   MaxPool. & 2x2 & None & 0 & ReLu \\
 \hline
 Fc. & - & - & - & Sigmoid \\
 \hline
        \end{tabular}
        
    \end{subtable}
    \caption{FoCNN feature extractors.}
\end{table}

\subsection{Postprocessing}
The output of neural networks are probabilities from 0 to 1. We determine a threshold to predict a source deduced from the results on the validation data. We search for $k$ which gives a threshold $\mu(x) + k*\sigma(x)$ minimizing the metrics score. Here $\mu(x)$ is an average over all pixels and $\sigma(x)$ is a deviation over all pixels across an image $x$. Via optimization on the validation set, we found $k$ equal to 25. So for each picture, we determine its own threshold.

To increase precision during the prediction stage, we crop images with intersections. All predictions are averaged across each pixel. It results in the fading of sources that are not sustained to shifting.

If sources are predicted in two neighboring pixels, we return only one of them corresponding to the maximum score assigned by the neural network.

==> relatedwork/relatedwork.tex <==


\section{Related Work}
\label{sec:related_work}
There are many algorithms for solving the deconvolution problem. In the optics range, one of the first algorithms is CLEAN by \cite{clean}. It works in Fourier inverse image space and removes source by source. One of the most well-known heuristic methods is SExtractor by \cite{sxtractor1996}. This algorithm analyses an astrophysical image in the following stages: a) the algorithm estimates a background level and constructs the background map, b) detecting object via thresholding, and peak finding methods c) detected objects are checked and separated, if necessary, d) algorithm cleans spurious detections and estimates the total magnitude of found objects e) neural network classifies point-like sources. Nevertheless, SExtractor returns only the list of point sources without denoised and deconvolved signal. 


The probabilistic approach describes the probabilistic relations between the data and the sources. Powellsnakes by \cite{powellsnakes} is an algorithm for detecting objects on multi-frequency astronomical images based on the Bayesian filters that use a prior for position, size, number of sources, flux, and spectral parameters. It uses PSF templates for detection and classification. However, no implementation of this approach is available, so we exclude it from our comparison. Another probabilistic method is D3PO by \cite{d3po} that aims at the concurrent denoising, deconvolution, and decomposition of photon observation into two components: the diffuse component, and point-like photon sources. This algorithm uses Bayesian inference and is based on the difference between the intensity of the source component and the cosmic background. 

D3PO reconstructs the diffused and point-like photon flux from a single photon count image. The method does not distinguish between diffuse sources and background, and both are considered to be the diffuse contribution. The method is based on several predetermined well-known prior distributions. 

Convolution neural networks (CNN) are currently one of the most powerful and accurate image processing algorithms available. CNNs are widespread in image processing tasks spanning from the recognition of handwritten digits by \cite{lenet} to the analysis of the complex medical images by \cite{brain}. Recently this approach has been applied to the domain of optical astrophysical analysis.  \cite{fermi_cnn}, describes the process of astrophysical image reconstruction using leNet-like architecture. \cite{gan} introduce the method of restoring astrophysical images using Generative Adversarial Networks which enable recovering features from heavily noised images.


==> results/res.tex <==
\section{Results}
We present the results of the comparison of D3PO, SExtractor, YOLO, CNN, Unet and FoCNN in the Table \ref{table:summary}. We characterise the performance of each algorithm by its F1 score, true-positive rate, metrics score, variation of metrics and a testing time for one picture $200 \times 200$ pixels. Metrics score in this table is a mean of all scores in the data set. Variation is also computed over all the data set. We specify that testing time includes only optimization step without post processing. The predicted point is considered true positive if it is contained in a circle with a radius of 1.6 pixels from the real point source which corresponds to the Fermi/LAT characteristic sources localization accuracy of $0.1^\circ$.



\begin{center}
\begin{table}
\centering
\makebox[0pt][c]{\parbox{0.9\textwidth}
{
\begin{minipage}[b]{1.0\linewidth}\centering
 \begin{tabular}{|| c || c | c | c | c | c ||}
 \hline
 & f1 & TPR  & Mean(\rho) & Var(\rho) & $t_\text{test}$ \\[0.5ex]
 \hline\hline
 D3PO & 0.45 & 0.31 & 402 & 227 &  \textgreater 10^6 ms\\

 \hline
 SExtractor & 0.49 & 0.36 & 346 & 223 & 236 ms\\
 \hline
 CNN & 0.49 & 0.36 & 376 & 217 & \bf{34 ms}\\
    \hline
 YOLO & 0.48 & 0.38 & 341 & 185 & 41 ms\\
 \hline
 UNet &  \bf{0.55} & 0.38 & 300 & 188 & 44 ms \\
 \hline
 
 FoCNN &  \bf{0.55} &  \bf{0.40} &  \bf{298} &  \bf{187} & 51 ms\\
 \hline
\end{tabular}
\end{minipage}\hfill
}}\vspace*{2mm}
\caption{A summary table for test set. F1 and TPR scores are computed for 0.1 degree radius which corresponds to standard Fermi Telescope error (1.6 pixels). If a predicted sources is found within this distance from the original one, the prediction is considered to be correct. $\rho$ is the value of the metrics described in Subsection \ref{desc:metrics}. Mean and Variance are taken over all images from the test set.  $t_\text{test}$ corresponds to an average execution time for one image from the test set.}
\label{table:summary}
\end{table}
\end{center}



%Empirically, it was found that the most important parameters are:
%DETECT_MAXAREA =  24  
%DETECT_MINAREA =  1.85
%DETECT_THRESH = 1.85 
%ANALYSIS_THRESH = 20000


%\begin{figure}
%    \centering
%    \includegraphics[scale=0.25]{images/predict.png}
%    \caption{UNet model predictions on test data.}
%    \label{fig:predit}
%\end{figure}


%In the figure \ref{fig:predit} we present examples of UNet outputs. The sources on the left and right are well recognized by the network, but in the middle model misses many of them. Such behavior is confirmed by the metrics.

% razdelit d3po slow and so on, 
% experiments on which data and describe in text the table (for those who in the tank)


